Dark Energy Survey Year 3 Results: Deep Field Optical + Near-Infrared Images and Catalogue

We describe the Dark Energy Survey (DES) Deep Fields, a set of images and associated multi-wavelength catalogue ($ugrizJHKs$) built from Dark Energy Camera (DECam) and Visible and Infrared Survey Telescope for Astronomy (VISTA) data. The DES Deep Fields comprise 11 fields (10 DES supernova fields plus COSMOS), with a total area of $\sim30~$ square degrees in $ugriz$ bands and reaching a maximum $i$-band depth of 26.75 (AB, $10\sigma$, 2 arcsec). We present a catalogue for the DES 3-year cosmology analysis of those four fields with full 8-band coverage, totalling $5.88~$ sq. deg. after masking. Numbering $2.8~$million objects ($1.6~$million post masking), our catalogue is drawn from images coadded to consistent depths of $r=25.7, i=25, z=24.3$ mag. We use a new model-fitting code, built upon established methods, to deblend sources and ensure consistent colours across the $u$-band to $Ks$-band wavelength range. We further detail the tight control we maintain over the point-spread function modelling required for the model fitting, astrometry and consistency of photometry between the four fields. The catalogue allows us to perform a careful star-galaxy separation and produces excellent photometric redshift performance (${\rm NMAD} = 0.023$ at $i<23$). The Deep-Fields catalogue will be made available as part of the cosmology data products release, following the completion of the DES 3-year weak lensing and galaxy clustering cosmology work.

==> DES-2020-0530_author_list_ordered.tex <==
% Author list file generated with: mkauthlist 1.2.4 
% mkauthlist --sort -j mnras --aux deepfields_authororder.csv DES-2020-0530_author_list.csv DES-2020-0530_author_list_ordered.tex 

\author[DES Collaboration]{
\parbox{\textwidth}{
\Large
W.~G.~Hartley,$^{1}$
A.~Choi,$^{2}$
A.~Amon,$^{3}$
R.~A.~Gruendl,$^{4,5}$
E.~Sheldon,$^{6}$
I.~Harrison,$^{7,8}$
G.~M.~Bernstein,$^{9}$
I.~Sevilla-Noarbe,$^{10}$
B.~Yanny,$^{11}$
K.~Eckert,$^{9}$
H.~T.~Diehl,$^{11}$
A.~Alarcon,$^{12}$
M.~Banerji,$^{13,14}$
K.~Bechtol,$^{15}$
S.~Cantu,$^{16}$
C.~Conselice,$^{8,17}$
S.~Everett,$^{18}$
D.~Gruen,$^{19,3,20}$
M.~Jarvis,$^{9}$
M.~D.~Johnson,$^{5}$
N.~MacCrann,$^{21}$
J.~Myles,$^{19,3,20}$
E.~S.~Rykoff,$^{3,20}$
C.~S{\'a}nchez,$^{9}$
F.~Tarsitano,$^{22}$
M.~A.~Troxel,$^{23}$
R.~Buchs,$^{20}$
J.~Cordero,$^{8}$
M.~E.~S.~Pereira,$^{24}$
C.~Davis,$^{3}$
T.~M.~Davis,$^{25}$
S.~Dodelson,$^{26}$
A.~Fert\'e,$^{27}$
K.~Honscheid,$^{2,28}$
N.~Kokron,$^{19,3}$
M.~Rodriguez-Monroy,$^{10}$
A.~B.~Pace,$^{26}$
A.~Palmese,$^{11,29}$
F.~Paz-Chinch\'{o}n,$^{13,5}$
A.~A.~Plazas,$^{30}$
J.~Prat,$^{31}$
S.~Samuroff,$^{26}$
L.~F.~Secco,$^{9}$
A.~Tong,$^{23}$
Z.~Vasquez,$^{26}$
A.~Drlica-Wagner,$^{31,11,29}$
C.~Zhou,$^{23}$
T.~M.~C.~Abbott,$^{32}$
M.~Aguena,$^{33,34}$
S.~Allam,$^{11}$
J.~Annis,$^{11}$
D.~Bacon,$^{35}$
E.~Bertin,$^{36,37}$
S.~Bhargava,$^{38}$
D.~Brooks,$^{39}$
D.~L.~Burke,$^{3,20}$
A.~Carnero~Rosell,$^{40,41}$
M.~Carrasco~Kind,$^{4,5}$
J.~Carretero,$^{42}$
F.~J.~Castander,$^{43,44}$
M.~Costanzi,$^{45,46}$
M.~Crocce,$^{43,44}$
L.~N.~da Costa,$^{34,47}$
J.~De~Vicente,$^{10}$
J.~DeRose,$^{48,18}$
S.~Desai,$^{49}$
J.~P.~Dietrich,$^{50}$
T.~F.~Eifler,$^{51,27}$
J.~Elvin-Poole,$^{2,28}$
I.~Ferrero,$^{52}$
B.~Flaugher,$^{11}$
P.~Fosalba,$^{43,44}$
J.~Garc\'ia-Bellido,$^{53}$
E.~Gaztanaga,$^{43,44}$
D.~W.~Gerdes,$^{54,24}$
J.~Gschwend,$^{34,47}$
G.~Gutierrez,$^{11}$
S.~R.~Hinton,$^{25}$
D.~L.~Hollowood,$^{18}$
D.~Huterer,$^{24}$
D.~J.~James,$^{55}$
S.~Kent,$^{11,29}$
E.~Krause,$^{51}$
K.~Kuehn,$^{56,57}$
N.~Kuropatkin,$^{11}$
O.~Lahav,$^{39}$
H.~Lin,$^{11}$
M.~A.~G.~Maia,$^{34,47}$
M.~March,$^{9}$
J.~L.~Marshall,$^{16}$
P.~Martini,$^{2,58,59}$
P.~Melchior,$^{30}$
F.~Menanteau,$^{4,5}$
R.~Miquel,$^{60,42}$
J.~J.~Mohr,$^{50,61}$
R.~Morgan,$^{15}$
E.~Neilsen,$^{11}$
R.~L.~C.~Ogando,$^{34,47}$
S.~Pandey,$^{9}$
A.~K.~Romer,$^{38}$
A.~Roodman,$^{3,20}$
M.~Sako,$^{9}$
E.~Sanchez,$^{10}$
V.~Scarpine,$^{11}$
S.~Serrano,$^{43,44}$
M.~Smith,$^{62}$
M.~Soares-Santos,$^{24}$
E.~Suchyta,$^{63}$
M.~E.~C.~Swanson,$^{5}$
G.~Tarle,$^{24}$
D.~Thomas,$^{35}$
C.~To,$^{19,3,20}$
T.~N.~Varga,$^{61,64}$
A.~R.~Walker,$^{32}$
W.~Wester,$^{11}$
R.D.~Wilkinson,$^{38}$
and J.~Zuntz$^{65}$
\begin{center} (DES Collaboration) \end{center}
}
\vspace{0.4cm}
\\
\parbox{\textwidth}{
%\scriptsize
$^{1}$ D\'{e}partement de Physique Th\'{e}orique and Center for Astroparticle Physics, Universit\'{e} de Gen\`{e}ve, 24 quai Ernest Ansermet, CH-1211 Geneva, Switzerland\\
$^{2}$ Center for Cosmology and Astro-Particle Physics, The Ohio State University, Columbus, OH 43210, USA\\
$^{3}$ Kavli Institute for Particle Astrophysics \& Cosmology, P. O. Box 2450, Stanford University, Stanford, CA 94305, USA\\
$^{4}$ Department of Astronomy, University of Illinois at Urbana-Champaign, 1002 W. Green Street, Urbana, IL 61801, USA\\
$^{5}$ National Center for Supercomputing Applications, 1205 West Clark St., Urbana, IL 61801, USA\\
$^{6}$ Brookhaven National Laboratory, Bldg 510, Upton, NY 11973, USA\\
$^{7}$ Department of Physics, University of Oxford, Denys Wilkinson Building, Keble Road, Oxford OX1 3RH, UK\\
$^{8}$ Jodrell Bank Center for Astrophysics, School of Physics and Astronomy, University of Manchester, Oxford Road, Manchester, M13 9PL, UK\\
$^{9}$ Department of Physics and Astronomy, University of Pennsylvania, Philadelphia, PA 19104, USA\\
$^{10}$ Centro de Investigaciones Energ\'eticas, Medioambientales y Tecnol\'ogicas (CIEMAT), Madrid, Spain\\
$^{11}$ Fermi National Accelerator Laboratory, P. O. Box 500, Batavia, IL 60510, USA\\
$^{12}$ Argonne National Laboratory, 9700 South Cass Avenue, Lemont, IL 60439, USA\\
$^{13}$ Institute of Astronomy, University of Cambridge, Madingley Road, Cambridge CB3 0HA, UK\\
$^{14}$ Kavli Institute for Cosmology, University of Cambridge, Madingley Road, Cambridge CB3 0HA, UK\\
$^{15}$ Physics Department, 2320 Chamberlin Hall, University of Wisconsin-Madison, 1150 University Avenue Madison, WI  53706-1390\\
$^{16}$ George P. and Cynthia Woods Mitchell Institute for Fundamental Physics and Astronomy, and Department of Physics and Astronomy, Texas A\&M University, College Station, TX 77843,  USA\\
$^{17}$ University of Nottingham, School of Physics and Astronomy, Nottingham NG7 2RD, UK\\
$^{18}$ Santa Cruz Institute for Particle Physics, Santa Cruz, CA 95064, USA\\
$^{19}$ Department of Physics, Stanford University, 382 Via Pueblo Mall, Stanford, CA 94305, USA\\
$^{20}$ SLAC National Accelerator Laboratory, Menlo Park, CA 94025, USA\\
$^{21}$ Department of Applied Mathematics and Theoretical Physics, University of Cambridge, Cambridge CB3 0WA, UK\\
$^{22}$ Department of Physics, ETH Zurich, Wolfgang-Pauli-Strasse 16, CH-8093 Zurich, Switzerland\\
$^{23}$ Department of Physics, Duke University Durham, NC 27708, USA\\
$^{24}$ Department of Physics, University of Michigan, Ann Arbor, MI 48109, USA\\
$^{25}$ School of Mathematics and Physics, University of Queensland,  Brisbane, QLD 4072, Australia\\
$^{26}$ Department of Physics, Carnegie Mellon University, Pittsburgh, Pennsylvania 15312, USA\\
$^{27}$ Jet Propulsion Laboratory, California Institute of Technology, 4800 Oak Grove Dr., Pasadena, CA 91109, USA\\
$^{28}$ Department of Physics, The Ohio State University, Columbus, OH 43210, USA\\
$^{29}$ Kavli Institute for Cosmological Physics, University of Chicago, Chicago, IL 60637, USA\\
$^{30}$ Department of Astrophysical Sciences, Princeton University, Peyton Hall, Princeton, NJ 08544, USA\\
$^{31}$ Department of Astronomy and Astrophysics, University of Chicago, Chicago, IL 60637, USA\\
$^{32}$ Cerro Tololo Inter-American Observatory, NSF's National Optical-Infrared Astronomy Research Laboratory, Casilla 603, La Serena, Chile\\
$^{33}$ Departamento de F\'isica Matem\'atica, Instituto de F\'isica, Universidade de S\~ao Paulo, CP 66318, S\~ao Paulo, SP, 05314-970, Brazil\\
$^{34}$ Laborat\'orio Interinstitucional de e-Astronomia - LIneA, Rua Gal. Jos\'e Cristino 77, Rio de Janeiro, RJ - 20921-400, Brazil\\
$^{35}$ Institute of Cosmology and Gravitation, University of Portsmouth, Portsmouth, PO1 3FX, UK\\
$^{36}$ CNRS, UMR 7095, Institut d'Astrophysique de Paris, F-75014, Paris, France\\
$^{37}$ Sorbonne Universit\'es, UPMC Univ Paris 06, UMR 7095, Institut d'Astrophysique de Paris, F-75014, Paris, France\\
$^{38}$ Department of Physics and Astronomy, Pevensey Building, University of Sussex, Brighton, BN1 9QH, UK\\
$^{39}$ Department of Physics \& Astronomy, University College London, Gower Street, London, WC1E 6BT, UK\\
$^{40}$ Instituto de Astrofisica de Canarias, E-38205 La Laguna, Tenerife, Spain\\
$^{41}$ Universidad de La Laguna, Dpto. Astrofisica, E-38206 La Laguna, Tenerife, Spain\\
$^{42}$ Institut de F\'{\i}sica d'Altes Energies (IFAE), The Barcelona Institute of Science and Technology, Campus UAB, 08193 Bellaterra (Barcelona) Spain\\
$^{43}$ Institut d'Estudis Espacials de Catalunya (IEEC), 08034 Barcelona, Spain\\
$^{44}$ Institute of Space Sciences (ICE, CSIC),  Campus UAB, Carrer de Can Magrans, s/n,  08193 Barcelona, Spain\\
$^{45}$ INAF-Osservatorio Astronomico di Trieste, via G. B. Tiepolo 11, I-34143 Trieste, Italy\\
$^{46}$ Institute for Fundamental Physics of the Universe, Via Beirut 2, 34014 Trieste, Italy\\
$^{47}$ Observat\'orio Nacional, Rua Gal. Jos\'e Cristino 77, Rio de Janeiro, RJ - 20921-400, Brazil\\
$^{48}$ Department of Astronomy, University of California, Berkeley,  501 Campbell Hall, Berkeley, CA 94720, USA\\
$^{49}$ Department of Physics, IIT Hyderabad, Kandi, Telangana 502285, India\\
$^{50}$ Faculty of Physics, Ludwig-Maximilians-Universit\"at, Scheinerstr. 1, 81679 Munich, Germany\\
$^{51}$ Department of Astronomy/Steward Observatory, University of Arizona, 933 North Cherry Avenue, Tucson, AZ 85721-0065, USA\\
$^{52}$ Institute of Theoretical Astrophysics, University of Oslo. P.O. Box 1029 Blindern, NO-0315 Oslo, Norway\\
$^{53}$ Instituto de Fisica Teorica UAM/CSIC, Universidad Autonoma de Madrid, 28049 Madrid, Spain\\
$^{54}$ Department of Astronomy, University of Michigan, Ann Arbor, MI 48109, USA\\
$^{55}$ Center for Astrophysics $\vert$ Harvard \& Smithsonian, 60 Garden Street, Cambridge, MA 02138, USA\\
$^{56}$ Australian Astronomical Optics, Macquarie University, North Ryde, NSW 2113, Australia\\
$^{57}$ Lowell Observatory, 1400 Mars Hill Rd, Flagstaff, AZ 86001, USA\\
$^{58}$ Department of Astronomy, The Ohio State University, Columbus, OH 43210, USA\\
$^{59}$ Radcliffe Institute for Advanced Study, Harvard University, Cambridge, MA 02138\\
$^{60}$ Instituci\'o Catalana de Recerca i Estudis Avan\c{c}ats, E-08010 Barcelona, Spain\\
$^{61}$ Max Planck Institute for Extraterrestrial Physics, Giessenbachstrasse, 85748 Garching, Germany\\
$^{62}$ School of Physics and Astronomy, University of Southampton,  Southampton, SO17 1BJ, UK\\
$^{63}$ Computer Science and Mathematics Division, Oak Ridge National Laboratory, Oak Ridge, TN 37831\\
$^{64}$ Universit\"ats-Sternwarte, Fakult\"at f\"ur Physik, Ludwig-Maximilians Universit\"at M\"unchen, Scheinerstr. 1, 81679 M\"unchen, Germany\\
$^{65}$ Institute for Astronomy, University of Edinburgh, Edinburgh EH9 3HJ, UK\\
}
}

